The longlived charged massive scalar field in the higher-dimensional Reissner--Nordstr\"{o}m spacetime

The quasinormal resonance frequency of the higher-dimensional Reissner--Nordstr\"{o}m (RN) black hole due to charged massive scalar field perturbation is deduced analytically in the eikonal regime. The characteristic decay timescale of the charged massive scalar perturbation in the background of the higher-dimensional RN spacetime is then obtained. The result reveals that longlived charged massive scalar field can exist in higher-dimensional RN spacetime under a certain condition.

==> __latexindent_temp.tex <==
Mo:2018nnu
